Does the Proof Prove It That Way? Faithful Formalization of Elements Proofs

In formal verification, both the autoformalization of statements and automated proof search have been studied extensively. While automated proof search can produce a formal proof that compiles, the generated proof does not necessarily reflect how the natural-language argument arrives at its conclusion--a property we refer to as faithfulness. With faithfully formalized proofs, one can check the reasoning behind a human- or AI-written argument, and assist mathematicians in formalizing their proof sketches. However, it is particularly challenging due to misalignment of formal proof tactics and natural language reasoning. In this work, we rigorously describe a set of five necessary conditions a faithful formal proof must satisfy, and introduce Pistis, an agentic, oracle-guided proof search that produces formal Lean proofs that satisfy them. At its core is a novel faithfulness-preserving divide-and-conquer search, which we name OrderDecompose, that tracks citation dependencies and blocks unfaithful shortcuts, paired with a refutation search, that surfaces gaps and errors in the natural language proof source. OrderDecompose completes proofs that baselines cannot close even within a 12-hour budget, and its artifacts compile over 33$\times$ as fast as prior work's. We apply Pistis on the first three books of Euclid's Elements, producing high-quality artifacts containing faithful formal proofs. Under a blinded human study and an LLM-as-a-judge protocol on rigorous rubrics, Pistis-generated proofs are favored over prior works--2.89$\times$ and 5.2$\times$ as often by human reviewers and the LLM judge, respectively. It further uncovers gaps in Euclid's proofs and their translation, and can accept or refute natural language proofs written by humans or AI, demonstrating that faithful formalization is useful as a proof-checking tool.

==> figures/fig-accept-refute-body.tex <==
\setlength{\parindent}{0pt}
\newlength{\colw}\setlength{\colw}{0.214\textwidth}

% card title
\newcommand{\ctitle}[1]{%
  {\footnotesize\bfseries #1}\\[-7pt]%
  {\color{black!25}\rule{\linewidth}{0.4pt}}\par\vspace{0pt}}

\newsavebox{\nlbox}\newsavebox{\codebox}

% import SystemE
% import Book1.Prop32.Main

% set_option systemE.solverTime 30
% set_option linter.unusedVariables false
% set_option linter.unnecessarySeqFocus false

% namespace AcceptRefute
% open Elements.Book1

% theorem proposition_5 : ∀ (a b c d e : Point) (AB BC AC : Line),
%   formTriangle a b c AB BC AC ∧ (|(a─b)| = |(a─c)|) ∧
%   (between a b d) ∧ (between a c e) →
%   (∠ a:b:c = ∠ a:c:b) ∧ (∠ c:b:d = ∠ b:c:e) := by
%   euclid_intros
%   euclid_intro_sentence "1.5.0"
%     "For isosceles triangles, the angles at the base are equal to one another, and if the equal sides are produced then the angles under the base will be equal to one another. Let $ABC$ be an isosceles triangle having the side $AB$ equal to the side $AC$, and let the straight-lines $BD$ and $CE$ have been produced in a straight-line with $AB$ and $AC$ (respectively) [Post.~2]. I say that the angle $ABC$ is equal to $ACB$, and (angle) $CBD$  to $BCE$. "

%   -- @assumption ("the side $AB$ is equal to the side $AC$", |(a─b)| = |(a─c)|)
%   euclid_sentence "1.5.1"
%     "Since the side $AB$ is equal to the side $AC$, the base angles are equal to one another, so the angle $ABC$ is equal to the angle $ACB$."
%     (step1 : ∠ a:b:c = ∠ a:c:b) := by sorry

%   -- @assumption ("the points $A$, $B$, $D$ lie in a straight line", between a b d)
%   -- @assumption ("likewise $A$, $C$, $E$", between a c e)
%   euclid_sentence "1.5.2"
%     "And since the points $A$, $B$, $D$ lie in a straight line, and likewise $A$, $C$, $E$, the angle $ABC$ together with $CBD$ makes two right-angles, and the angle $ACB$ together with $BCE$ makes two right-angles."
%     (step2 : (∠ a:b:c + ∠ c:b:d = ∟ + ∟) ∧ (∠ a:c:b + ∠ b:c:e = ∟ + ∟)) := by sorry

%   euclid_sentence "1.5.3"
%     "Now the angle $CBD$ is itself a right-angle, since $BC$ stands upon the straight-line $AD$."
%     (step3 : ∠ c:b:d = ∟) := by sorry

%   have refute_step3 : ¬ (∠ c:b:d = ∟) := by
%     euclid_apply (proposition_32 c a b d AC AB BC)
%     euclid_finish

%   -- @contradiction
%   have contradiction : False := by
%     apply refute_step3 step3

%   euclid_sentence "1.5.4"
%     "And in the same way the angle $BCE$ is a right-angle."
%     (step4 : ∠ b:c:e = ∟) := by sorry

%   euclid_sentence "1.5.5"
%     "Therefore the angle $CBD$ is equal to the angle $BCE$, each being a right-angle."
%     (step5 : ∠ c:b:d = ∠ b:c:e) := by sorry

%   euclid_sentence "1.5.6"
%     "Thus, the angles at the base are equal to one another, and the angles under the base are equal to one another."
%     (step6 : (∠ a:b:c = ∠ a:c:b) ∧ (∠ c:b:d = ∠ b:c:e)) := by sorry

%   exact step6
%   euclid_conclude_sentence "1.5.7"
%     "(Which is) the very thing it was required to show."

% end AcceptRefute

\begin{lrbox}{\nlbox}
\begin{minipage}{\colw}
\ctitle{NL Source}
\scriptsize\linespread{0.85}\selectfont
\textbf{Prop~I-5.} For isosceles triangles, the angles at the base are equal to one another. and if the equal sides are\dots\\[0pt]
\textbf{Proof.}
Since the side $AB$ is equal to the side $AC$, the base angles are equal to one another\dots
{\color{sD} Now the angle $CBD$ is itself a right-angle \smark[sD]{3},}\dots
Which is the very thing required to show.
% \colorbox{sD!15}{%
%   \begin{minipage}{0.9\linewidth}
%     Since the side $AB$ is equal to the side $AC$, the base angles are equal to one another, so the angle $ABC$ is equal to the angle $ACB$.
%   \textcolor{sD!70!black}{\textbf{s3:} Now the angle $CBD$ is itself a right-angle}
%   \end{minipage}%
% }\\[0pt]
\end{minipage}
\end{lrbox}

\begin{lrbox}{\codebox}
\begin{minipage}{\colw}
\ctitle{Formal refutation}
\begin{lstlisting}[style=lean, mathescape=true, basicstyle=\ttfamily\fontsize{7}{7.4}\selectfont]
theorem p5: ∀(a b c…) …
 → (∠c:b:d=∠b:c:e) := by
  have s3 : ∠ c:b:d = ∟
   := by sorry
  have refute_s3 :
   ¬(∠ c:b:d = ∟) := by
    …; euclid_finish
  have contra : False :=
   refute_s3 s3
\end{lstlisting}
\vspace{-2.5px}
\end{minipage}
\end{lrbox}

\begin{tikzpicture}[
  font=\footnotesize,
  card/.style={draw=black!55, rounded corners=2pt, line width=0.5pt,
               inner sep=4pt, anchor=north west},
  neutral/.style={card, fill=black!2},
]

\node[neutral] (nl) at (0,0) {\usebox{\nlbox}};
\node[neutral, anchor=north west] (code) at ($(nl.north east)+(2mm,0)$) {\usebox{\codebox}};

% Highlight the `contra` block (listing lines 7--8): top of line 7 to bottom of line 8.
\pgfmathsetlengthmacro{\lineH}{7.72pt}
\pgfmathsetlengthmacro{\codeTop}{9.2pt}
\pgfmathsetlengthmacro{\stepThreeTop}{\codeTop+3*\lineH}
\pgfmathsetlengthmacro{\stepThreeBot}{\codeTop+5*\lineH}
\fill[sD, fill opacity=0.12, rounded corners=1.5pt]
  ([xshift=3pt, yshift=-\stepThreeTop]code.north west)
  rectangle ([xshift=-3pt, yshift=-\stepThreeBot]code.north east);

\node[font=\scriptsize, anchor=south east, inner sep=1pt]
    at ([xshift=-1.5pt, yshift=-\stepThreeBot]code.north east) {\smark[sD]{3}};

\pgfmathsetlengthmacro{\contraTop}{\codeTop+8*\lineH}
\pgfmathsetlengthmacro{\contraBot}{\codeTop+10*\lineH}
\fill[red, fill opacity=0.12, rounded corners=1.5pt]
  ([xshift=3pt, yshift=-\contraTop]code.north west)
  rectangle ([xshift=-3pt, yshift=-\contraBot]code.north east);

\end{tikzpicture}


==> figures/fig-accept-refute.tex <==
% =====================================================================
% Accept/Refute example (Book I, Prop 5 refutation).
% Illustrates: ∃i, Δ ∪ {α} ⊢ ¬formal(assert(s_i))
% Two narrow columns: NL proof excerpt + formal refutation
% =====================================================================
\begin{figure}[t]
\centering
\input{figures/fig-accept-refute-body.tex}
\vspace{-18px}
\caption{
  Formal refutation of an LLM-generated proof.
  \textit{Left:} excerpt from an LLM-generated proof with false claim $s_3$.
  \textit{Right:} we prove $\neg\formal{\assert{s_3}}$.
}
\label{fig:accept-refute}
% \vspace{-10px}
\end{figure}


==> figures/fig-citation-mistake-body.tex <==
\setlength{\parindent}{0pt}
\newlength{\colwB}\setlength{\colwB}{0.214\textwidth}

\newcommand{\ctitleB}[1]{%
  {\footnotesize\bfseries #1}\\[-4pt]%
  {\color{black!25}\rule{\linewidth}{0.4pt}}\par\vspace{0pt}}

\newsavebox{\nlboxB}\newsavebox{\codeboxB}\newsavebox{\pageboxB}

% 1.9 To cut a given rectilinear angle in half.
% 1.10 To cut a given finite straight-line in half.



% theorem proposition_1 : ∀ (ABC : Circle),
%   ∃ f : Point, f.isCentre ABC :=
% by
%   euclid_intros
%   euclid_intro_sentence "3.1.0"
%     "To find the center of a given circle. Let $ABC$ be the given circle. So it is required to find the center of circle $ABC$."

%   euclid_apply (exists_point_on_circle ABC) as a
%   euclid_apply (exists_distinct_point_on_circle ABC a) as b
%   euclid_apply (line_from_points a b) as AB
%   euclid_sentence "3.1.1"
%     "Let some straight-line $AB$ be drawn through ($ABC$), at random,"
%     (step1 : a.onCircle ABC ∧ b.onCircle ABC ∧ distinctPointsOnLine a b AB) := by euclid_apply (helper_3_1_step1 ABC a b AB (by euclid_assumption "" (show a.onCircle ABC; assumption)) (by euclid_assumption "" (show b.onCircle ABC; assumption)) (by euclid_assumption "" (show a.onLine AB; assumption)) (by euclid_assumption "" (show b.onLine AB; assumption)) (by euclid_assumption "" (show b ≠ a; assumption)))

%   euclid_apply (proposition_10 a b AB) as d
%   -- @suppress_deps_check "Source edition (Fitzpatrick) brackets this segment-bisection as [Prop.~1.9], but 1.9 is angle-bisection; bisecting a straight-line is I.10 — the faithful construction applies proposition_10. Editorial bracket typo in the source, not ours."
%   euclid_sentence "3.1.2"
%     "and let ($AB$) be cut in half at point $D$ [Prop.~1.9]."
%     (step2 : between a d b ∧ |(a─d)| = |(d─b)|) := by euclid_apply (helper_3_1_step2 a b d (by euclid_assumption "" (show between a d b; assumption)) (by euclid_assumption "" (show |(a─d)| = |(d─b)|; assumption)))
% ...
% end Elements.Book3

\begin{lrbox}{\nlboxB}
\begin{minipage}{\colwB}
\ctitleB{NL Source}
\scriptsize\linespread{0.85}\selectfont
\textbf{Prop III-1.} To find the center of a given circle. Let $ABC$ be the given circle\dots\\[0.7pt]
\textbf{Proof.}
Let some straight-line $AB$ be drawn through ($ABC$), at random \smark{1},
{\color{sD} and let ($AB$) be cut in half at point $D$ \refpill{Proposition I-9} \smark[sD]{2}}.
\dots
% \colorbox{sA!14}{%
%   \begin{minipage}{0.9\linewidth}
%   \textcolor{sA!80!black}{and let ($AB$) be cut in half at point $D$}
%   \colorbox{sC!18}{\textcolor{sC!80!black}{\textbf{[Prop.~I-9]}}}.
%   \end{minipage}%
% }\\[0pt]
% {\color{black!25}\rule{\linewidth}{0.4pt}}\\[0pt]
% \textbf{Prop.~I-9.}~cut...
% \colorbox{sC!18}{\textcolor{sC!80!black}{\textbf{angle}}} in half.\\
% \textbf{Prop.~I-10.}~cut...
% \colorbox{sB!18}{\textcolor{sB!80!black}{\textbf{straight-line}}}...
\end{minipage}
\end{lrbox}

\begin{lrbox}{\codeboxB}
\begin{minipage}{\colwB}
\ctitleB{Faithful formalization}
\begin{lstlisting}[style=lean, basicstyle=\ttfamily\fontsize{7}{7.4}\selectfont]
theorem p1: ∀(ABC: Circle),
 ∃f: Point, f.isCentre ABC
 := by …
  euclid_apply prop_10 …
  -- @suppress_deps_check
  have s2: between a d b
  ∧ |(a─d)|=|(d─b)|:= by…
\end{lstlisting}
\vspace{-3px}
\end{minipage}
\end{lrbox}

% ---- book-page excerpt (top): what I-9 and I-10 actually cut, with the key
%      words tinted to match the code highlights (angle=sC/orange, line=sB/green)
\begin{lrbox}{\pageboxB}
\begin{minipage}{\dimexpr2\colwB+2mm+8pt\relax}
\scriptsize\linespread{0.9}\selectfont
\textbf{Prop~I-9.}~To cut a given rectilinear {\setlength{\fboxsep}{1pt}\colorbox{sC!18}{\textcolor{sC!80!black}{angle}}} in half. Let $BAC$ be the given recti\dots \\
\textbf{Prop~I-10.}~To cut a given finite {\setlength{\fboxsep}{1pt}\colorbox{sB!18}{\textcolor{sB!80!black}{straight-line}}} in half. Let $AB$ be the given finite\dots
\end{minipage}
\end{lrbox}

\begin{tikzpicture}[
  font=\footnotesize,
  card/.style={draw=black!55, rounded corners=2pt, line width=0.5pt,
               inner sep=4pt, anchor=north west},
  neutral/.style={card, fill=black!2},
  bookpage/.style={draw=black!50, fill=white, line width=0.4pt,
                   inner sep=4pt, anchor=south west},
]

% book-page excerpt sits above the two cards, with a slight drop shadow
\node[bookpage] (page) at (0, 2.5mm) {\usebox{\pageboxB}};
\begin{scope}[on background layer]
  \fill[black!22] ([xshift=1.4pt, yshift=-1.4pt]page.north west)
                  rectangle ([xshift=1.4pt, yshift=-1.4pt]page.south east);
\end{scope}

\node[neutral] (nlB) at (0,0) {\usebox{\nlboxB}};
\node[neutral, anchor=north west] (codeB) at ($(nlB.north east)+(2mm,0)$) {\usebox{\codeboxB}};

% ---- highlight prop_10 (line 1, sB/green, matching the straight-line box)
%      and @suppress_deps_check (line 2, sC/orange, matching [Prop.~1.9]).
%      \codeTopB = card top -> top of code line 1; \lineHB = baselineskip.
\pgfmathsetlengthmacro{\lineHB}{7.48pt}
\pgfmathsetlengthmacro{\codeTopB}{20.2pt}
% line 1 -- prop_10 (sB/green)
\pgfmathsetlengthmacro{\propTop}{\codeTopB+(4-1)*\lineHB}
\pgfmathsetlengthmacro{\propBot}{\codeTopB+4*\lineHB}
\fill[sB, fill opacity=0.18, rounded corners=1.5pt]
  ([xshift=3pt, yshift=-\propTop]codeB.north west)
  rectangle ([xshift=-3pt, yshift=-\propBot]codeB.north east);
% line 2 -- @suppress_deps_check (orange)
\pgfmathsetlengthmacro{\supTop}{\codeTopB+(5-1)*\lineHB}
\pgfmathsetlengthmacro{\supBot}{\codeTopB+5*\lineHB}
\fill[sC, fill opacity=0.18, rounded corners=1.5pt]
  ([xshift=3pt, yshift=-\supTop]codeB.north west)
  rectangle ([xshift=-3pt, yshift=-\supBot]codeB.north east);
% lines 3-6 -- have step2 (blue, matching the "cut ... at D" phrase)
\pgfmathsetlengthmacro{\haveTop}{\codeTopB+(6-1)*\lineHB}
\pgfmathsetlengthmacro{\haveBot}{\codeTopB+7*\lineHB}
\fill[sD, fill opacity=0.14, rounded corners=1.5pt]
  ([xshift=3pt, yshift=-\haveTop]codeB.north west)
  rectangle ([xshift=-3pt, yshift=-\haveBot]codeB.north east);
\node[font=\scriptsize, anchor=north east, inner sep=1pt]
    at ([xshift=-1.5pt, yshift=-\haveTop]codeB.north east) {\smark[sD]{2}};


\end{tikzpicture}


==> figures/fig-citation-mistake.tex <==
% =====================================================================
% Citation-mistake example (Book III, Prop 1) -- compact.
% Source edition brackets the WRONG proposition; the step is TRUE, so we
% waive the dep check (@suppress_deps_check) instead of refuting.
% =====================================================================
\begin{figure}[t]
\centering
\input{figures/fig-citation-mistake-body.tex}
\vspace{-18px}
\caption{
  A citation gap unveiled in the proof of Prop. III-1.
  Fitzpatrick brackets ``cut $AB$ in half'' as \refpill{Proposition I-9}, but
  I-9 is about \emph{angles}, not straight lines, and it should be Prop~I-10.
}
\label{fig:citation-mistake}
\vspace{-2px}
\end{figure}


==> figures/fig-motivation-body.tex <==
\setlength{\parindent}{0pt}
% widths: the statement card spans \stmtw; the THREE proof cards below
% together span the SAME width (each \panelw + two 3mm gutters).
\newlength{\stmtw}\setlength{\stmtw}{0.65\textwidth}
\newlength{\panelw}\setlength{\panelw}{\dimexpr(\stmtw-16pt-6mm)/3\relax}
% The unfaithful and partly-faithful panels are narrowed; the width they give
% up goes to the faithful panel. The three deltas must cancel (-24-10+34=0) so
% the row still sums to 3*\panelw, i.e. exactly the statement card's width.
\newlength{\supw}\setlength{\supw}{\dimexpr\panelw-24pt\relax}
\newlength{\badw}\setlength{\badw}{\dimexpr\panelw-10pt\relax}
\newlength{\faiw}\setlength{\faiw}{\dimexpr\panelw+34pt\relax}
% Sentence-group colours (sA..sD), \cnum, and \smark are defined once in the
% preamble (main.tex) so the running text can use the same styling.

% card title: bold label + thin rule (\par-terminated so lstlisting can follow)
% \footnotesize is explicit so the boxed cards (built outside the tikzpicture,
% hence \normalsize) match the left Euclid card, which inherits the picture's
% font=\footnotesize. Changing this size shifts \codeTop -- retune it below.
\newcommand{\cardtitle}[1]{%
  {\footnotesize\bfseries #1}\\[-4pt]%
  {\color{black!25}\rule{\linewidth}{0.4pt}}\par\vspace{0pt}}

% ---- code panels: built into boxes first (lstlisting cannot sit inside a
%      tikz node argument), then placed with \usebox in the nodes below ----
\newsavebox{\stmtbox}\newsavebox{\supbox}\newsavebox{\badbox}\newsavebox{\faibox}

\begin{lrbox}{\stmtbox}
\begin{minipage}{\stmtw}
\cardtitle{Formal statement in Lean \normalfont\itshape(given)}
\begin{lstlisting}[style=lean]
theorem proposition_6 : ∀ (a b c : Point) (AB BC AC : Line),
  formTriangle a b c AB BC AC ∧ (∠ a:b:c = ∠ a:c:b) → |(a─b)| = |(a─c)|
\end{lstlisting}
\end{minipage}
\end{lrbox}

\begin{lrbox}{\supbox}
\begin{minipage}{\supw}
\cardtitle{Unfaithful}
\begin{lstlisting}[style=lean]
by
 euclid_intros
 euclid_apply
  (superposition
    a b c a c b
    AB BC AC AC)
  as
  (b',c',BC',AC')
 euclid_finish
\end{lstlisting}
\end{minipage}
\end{lrbox}

\begin{lrbox}{\badbox}
\begin{minipage}{\badw}
\cardtitle{Partly faithful}
\begin{lstlisting}[style=lean]
by euclid_intros
 by_contra
 by_cases
   |(a─b)| > |(a─c)|
 · -- the first case
   euclid_apply
    (prop_3 …) as d
   euclid_apply
    (line d c) as DC
   euclid_apply
    prop_4 …
   euclid_finish
 · -- the second case
   euclid_apply
    (prop_3 …) as d
   …
   euclid_finish
\end{lstlisting}
\end{minipage}
\end{lrbox}

\begin{lrbox}{\faibox}
\begin{minipage}{\faiw}
\cardtitle{Faithful \normalfont\itshape(ours)}
\begin{lstlisting}[style=lean]
by euclid_intros
 have habsurd:
  ¬(|(a─b)|≠|(a─c)|) := …
  wlog gt: |(a─b)| > |(a─c)|
   generalizing b c AB BC AC
   with Hsym
  · … -- prove symmetry gap
  · have s3: between b d a
     ∧ |(b─d)|=|(a─c)| := …
    … -- steps 4-5
    have s6: ∠d:b:c = ∠a:c:b
    … -- steps 7-9
 have s10: ¬(|(a─b)|≠|(a─c)|)
  := by exact habsurd
 have s11: |(a─b)| = |(a─c)|
  := by_contra …
 exact s11
\end{lstlisting}
\end{minipage}
\end{lrbox}

\begin{tikzpicture}[
  font=\footnotesize,
  card/.style={draw=black!55, rounded corners=2pt, line width=0.5pt,
               inner sep=4pt, anchor=north west},
  neutral/.style={card, fill=black!2},
  unfa/.style={card, fill=red!5, draw=red!50!black},     % completely unfaithful
  part/.style={card, fill=cBaseline!14, draw=cBaselineD}, % partly faithful (baseline: blue)
  ours/.style={card, fill=cMine!20, draw=cMineD},         % faithful (ours: gold)
]

% =====================  (A) Euclid original  ==========================
\node[neutral] (euclid) at (0,0) {%
  \begin{minipage}{0.30\textwidth}
  \cardtitle{Euclid, \emph{Elements}~I-6}
  % --- verbatim text from docs/comparison/original_text.tex ---
  % markers \smark{k} sit exactly at the sentence splits used by the
  % faithful proof (tags "1.6.k"); references become \refpill{...}.
  \textbf{Statement.}
  If a triangle has two angles equal to one another then the sides subtending the equal angles will also be equal to one another.
  Let $ABC$ be a triangle having the angle $ABC$ equal to the angle $ACB$.
  I say that side $AB$ is also equal to side $AC$.\\[3pt]
  \textbf{Proof.}
  \textcolor{sA}{For if $AB$ is unequal to $AC$ then one of them is greater.\smark[sA]{1}}
  \textcolor{sA}{Let $AB$ be greater.\smark[sA]{2}}
  \textcolor{sB}{And let $DB$, equal to the lesser $AC$, have been cut off from the greater $AB$ \refpill{Proposition I-3}.\smark[sB]{3}}
  % And let $DC$ have been joined \refpill{Postulate 1}.\smark{4}
  % Therefore, since $DB$ is equal to $AC$, and $BC$ (is) common, the two sides $DB$, $BC$ are equal to the two sides $AC$, $CB$, respectively,\smark{5}
  Therefore, \dots,
  \textcolor{sC}{and the angle $DBC$ is equal to the angle $ACB$.\smark[sC]{6}}
  Thus, the base $DC$ is equal to the base $AB$,\smark{7}
  and the triangle $DBC$ will be equal to the triangle $ACB$ \refpill{Proposition I-4}, the lesser to the greater.\smark{8}
  The very notion (is) absurd \refpill{Common Notion 5}.\smark{9}
  \textcolor{sD}{Thus, $AB$ is not unequal to $AC$.\smark[sD]{10}}
  \textcolor{sD}{Thus, (it is) equal.\smark[sD]{11}}
  Thus, if a triangle has\dots\smark{12}
  % Thus, if a triangle has two angles equal to one another then the sides subtending the equal angles will also be equal to one another. (Which is) the very thing it was required to show.\smark{12}
  \unskip\nobreak\hfill$\square$
  \end{minipage}%
};

% =====================  (B) formal statement  ========================
\node[neutral, anchor=north west] (stmt) at ($(euclid.north east)+(3mm,0)$)
  {\usebox{\stmtbox}};

% =====================  (C1) unfaithful: superposition  ==============
\node[unfa, anchor=north west] (sup) at ($(stmt.south west)+(0,-3mm)$)
  {\usebox{\supbox}};

% =====================  (C2) partly faithful: prior work  ============
\node[part, anchor=north west] (bad) at ($(sup.north east)+(3mm,0)$)
  {\usebox{\badbox}};

% =====================  (C3) faithful (ours)  ========================
\node[ours, anchor=north west] (fai) at ($(bad.north east)+(3mm,0)$)
  {\usebox{\faibox}};

% ---- the I.6 diagram, in a callout pointing back into the left card -----
% Fills the empty space under the (short) Unfaithful card. Isosceles: AB=AC,
% so A sits horizontally centred above BC; D is on AB nearer A, DC dashed.
%
% ===== CALLOUT GEOMETRY -- every handle is a plain number, edit freely =====
%   \figDX/\figDY  position of the box's TOP-LEFT corner, measured from the
%                  bottom-left corner of the Unfaithful card
%                  (\figDX = right, \figDY = down).
%   \figW/\figH    exact box width and height (inner sep is 0, so these are
%                  the real outer dimensions; the diagram is centred inside).
%   \figPX/\figPY  the pointer TIP, measured from the left card's right edge
%                  at the height of the box's top (\figPX negative = further
%                  INTO the left card, \figPY = down).
%   \figPW         width of the pointer where it meets the box.
\newlength{\figDX}\setlength{\figDX}{0pt}
\newlength{\figDY}\setlength{\figDY}{7pt}
\newlength{\figW}\setlength{\figW}{82pt}
% NB: the free space under the Unfaithful card is ~60pt. Growing \figH past
% that makes the whole figure taller, which can bump the float to a later page.
\newlength{\figH}\setlength{\figH}{56pt}
\newlength{\figPX}\setlength{\figPX}{-4pt}
\newlength{\figPY}\setlength{\figPY}{47pt}
\newlength{\figPW}\setlength{\figPW}{7pt}
%   \figScale      size of the triangle diagram (pure number).
%   \figCX/\figCY  nudge the diagram inside the box, from its centre
%                  (\figCX = right, \figCY = up).
% The diagram is drawn OUTSIDE the callout node (see below), so changing any
% of these three can never alter the box geometry above.
\newcommand{\figScale}{0.70}
\newlength{\figCX}\setlength{\figCX}{0pt}
\newlength{\figCY}\setlength{\figCY}{-3pt}
% ==========================================================================
\coordinate (figanchor) at ($(sup.south west)+(\figDX,-\figDY)$);
\node[rectangle callout, anchor=north west,
      minimum width=\figW, minimum height=\figH, inner sep=0pt,
      callout absolute pointer={($(euclid.east|-figanchor)+(\figPX,-\figPY)$)},
      callout pointer width=\figPW,
      draw=black!55, fill=white, line width=0.5pt]
     (fig) at (figanchor) {};   % <-- deliberately EMPTY: see below

% The triangle is drawn as a normal part of the picture, merely *positioned*
% at the callout's centre. Because it is not the node's content, its size has
% no influence on the callout box -- the box stays exactly \figW x \figH.
% Coordinates are centred on the origin; AB=AC, so A is horizontally centred
% above BC, D sits on AB nearer A, and DC is dashed.
\begin{scope}[shift={($(fig.center)+(\figCX,\figCY)$)}, scale=\figScale,
              line width=0.5pt]
  \coordinate (Bp) at (-1,-0.78);
  \coordinate (Cp) at ( 1,-0.78);
  \coordinate (Ap) at ( 0, 0.88);
  \coordinate (Dp) at ($(Ap)!0.34!(Bp)$);
  \draw (Ap) -- (Bp) -- (Cp) -- cycle;
  \draw[dashed] (Dp) -- (Cp);
  % equal-angle arcs: angle ABC (rays BC->BA) and angle ACB (rays CB->CA).
  % AB=AC so the triangle is symmetric; the two sweeps mirror about the axis.
  \draw ([shift=(0:0.30)]Bp)     arc (0:58.9:0.30);
  \draw ([shift=(121.1:0.30)]Cp) arc (121.1:180:0.30);
  \foreach \p in {Ap,Bp,Cp,Dp}{\fill (\p) circle (0.06);}
  \node[font=\scriptsize, above=-1pt]       at (Ap) {$A$};
  \node[font=\scriptsize, below left=-3pt]  at (Bp) {$B$};
  \node[font=\scriptsize, below right=-3pt] at (Cp) {$C$};
  \node[font=\scriptsize, left=0pt]         at (Dp) {$D$};
\end{scope}

% ---- ANNOTATION (style draft): blue bar beside lines 2--5 of the
%      partly-faithful proof, echoing sentences (1)(2) [colour sA] ----
% Offsets are relative to the card's top-left; \lineH is the code
% baselineskip (matches the lean style's 7.8pt). Tune \barTop until the
% bar lines up with the code lines.
% code geometry inside the partly-faithful card (line 1 = "by")
\pgfmathsetlengthmacro{\lineH}{8.2pt}     % code baselineskip
\pgfmathsetlengthmacro{\codeTop}{20.2pt}  % card top -> top of line 1
\newlength{\annPadL}\setlength{\annPadL}{5pt} % shade left edge + bar inset
\newlength{\annPadR}\setlength{\annPadR}{1pt} % shade right edge inset
% \proofshade{node}{colour}{first}{last}: translucent shaded rectangle over the
% given (full-width) code lines of proof card <node>, plus a solid vertical bar
% on its left edge. Leaves \tmptop set for the label. Assumes the card uses the
% title + lean-listing layout, so \codeTop/\lineH apply (line 1 = "by").
\newcommand{\proofshade}[4]{%
  \pgfmathsetlengthmacro{\tmptop}{\codeTop+(#3-1)*\lineH}%
  \pgfmathsetlengthmacro{\tmpbot}{\codeTop+#4*\lineH}%
  \fill[#2, fill opacity=0.12, rounded corners=1.5pt]
    ([xshift=\annPadL, yshift=-\tmptop]#1.north west)
    rectangle ([xshift=-\annPadR, yshift=-\tmpbot]#1.north east);
  \draw[#2, line width=1.4pt, line cap=round]
    ([xshift=\annPadL, yshift=-\tmptop]#1.north west) --
    ([xshift=\annPadL, yshift=-\tmpbot]#1.north west);%
}
% \proofbar: label INSIDE the top-right corner (default -- use when the first
% line's right side is empty).
\newcommand{\proofbar}[5]{%
  \proofshade{#1}{#2}{#3}{#4}%
  \node[text=#2, font=\scriptsize, anchor=north east, inner sep=1pt]
    at ([xshift=-1.5pt, yshift=-\tmptop]#1.north east) {#5};%
}
% \proofbarT: label just ABOVE the filled area (use when the first line's text
% reaches the right edge and would collide with a corner label).
\newcommand{\proofbarT}[5]{%
  \proofshade{#1}{#2}{#3}{#4}%
  \node[text=#2, font=\scriptsize, anchor=south east, inner sep=1pt]
    at ([xshift=-1.5pt, yshift=-\tmptop]#1.north east) {#5};%
}
\proofbar{bad}{sA}{2}{4}{\cnum{sA}{1}\,\cnum{sA}{2}}
\proofbar{bad}{sB}{6}{9}{\cnum{sB}{3}}
\proofbar{fai}{sA}{2}{6}{\cnum{sA}{1}\,\cnum{sA}{2}}
\proofbar{fai}{sB}{8}{9}{\cnum{sB}{3}}
\proofbar{fai}{sC}{11}{11}{\cnum{sC}{6}}
\proofbarT{fai}{sD}{13}{16}{\cnum{sD}{10}--\cnum{sD}{11}}

% ---- flow annotations left as TODO ---------------------------------
% Gutters are ~3mm, too tight for labeled arrows.  Candidate relations:
%   Euclid card --"formalize"--> statement;  statement --"fill"--> proofs
%   Euclid sentence (k) <--> faithful step "1.6.k"  (needs per-line anchors)

\end{tikzpicture}


==> figures/fig-motivation.tex <==
% =====================================================================
% Motivating-example figure (Book I, Prop 6).
% Three cards, full width:
%   (A) left  : Euclid's original statement + NL proof, verbatim, with
%               superscript markers \smark{k} at the faithful-proof
%               sentence splits and \refpill{...} citation pills.
%   (B) top-right : the given formal Lean STATEMENT (spans right region)
%   (C) bottom-right, two panels:
%         (C1) a proof that merely COMPILES but is not faithful (prior work)
%         (C2) our FAITHFUL proof (each NL sentence -> one formal step)
% Code panels are real lstlisting (language=Lean, style defined in main.tex).
% Source: docs/comparison/{original_text.tex, Old_Prop06.lean, My_Prop06/Main.lean}
%
% Widths tuned to fit \textwidth: left 0.40 + right region ~0.56.
% If you change the left width, re-tune stmt (0.54) and panel (0.255) widths.
% =====================================================================
\begin{figure*}[ht]
\centering
\input{figures/fig-motivation-body.tex}
\caption{
  Motivating example (Book~I, Prop.~6).
  \textbf{Left:} Euclid's statement and natural-language proof, its sentences marked \smark{1}--\smark{12} at the points where our method splits them;
  citations appear as pills (e.g.\ \refpill{Proposition I-3});
  the accompanied diagram illustrates the corresponding geometric constructions.
  \textbf{Top right:} the formal statement we are given in Lean.
  \textbf{Bottom right:} three ways to fill the proof, from unfaithful to faithful.
  Left: a single \texttt{superposition} that discards Euclid's argument;
  middle: prior work~\cite{murphy_autoformalizing_2024}, where one \texttt{euclid\_finish} collapses many of Euclid's sentences;
  and right: our \emph{faithful} proof, where each NL sentence maps to exactly one formal step matching \smark{k} on the left.
}
\label{fig:motivation}
\vspace{-10px}
\end{figure*}


==> figures/fig-segment-body.tex <==
% matched-bracket colours: each open/close pair of the nested proof-term
% parens gets the same colour, so the trailing ))) is easy to read.
\definecolor{brkone}{RGB}{200,40,40}     % euclid_apply's argument
\definecolor{brktwo}{RGB}{40,110,200}    % h_step1's assumption argument
\definecolor{brkthree}{RGB}{200,120,0}   % e_assump's show argument
\providecommand{\lp}[1]{\textcolor{#1}{\bfseries(}}
\providecommand{\rp}[1]{\textcolor{#1}{\bfseries)}}
\begin{lstlisting}[style=lean, frame=single, framesep=4pt,
  rulecolor=\color{green!45!black}, backgroundcolor=\color{green!6},
  xleftmargin=2pt, xrightmargin=2pt, breaklines=false, escapechar=?,
  basicstyle=\ttfamily\fontsize{8.5}{10.5}\selectfont]
have step1_assumption1 : |(a─b)| ≠ |(a─c)| := by
  euclid_sentence "For if $AB$ is unequal to $AC$ then one of them is greater."
  (step1 : |(a─b)| > |(a─c)| ∨ |(a─c)| > |(a─b)|) :=
  by euclid_apply ?\lp{brkone}?helper_step1 … ?\lp{brktwo}?e_assump "$AB$ is unequal to $AC$" ?\lp{brkthree}?show |(a─b)| ≠ |(a─c)|; …?\rp{brkthree}??\rp{brktwo}??\rp{brkone}?
\end{lstlisting}


==> figures/fig-segment-img.tex <==
% Image-based: body compiled to vector PDF (fig-segment-standalone.pdf) with
% roboto-mono (Type-1). Caption/label stay LaTeX-set. Rebuild the vector PDF:
%   cd figures && TEXINPUTS="..:" pdflatex fig-segment-standalone.tex
\begin{figure*}[t]
\centering
\includegraphics{figures/fig-segment-standalone.pdf}
\caption{
  A single \emph{faithful step}: Euclid's sentence \smark{1} of Prop.~6, expanding from the same Prop~6 example from \cref{fig:motivation} which was a \emph{simplification}.
  This example uses \texttt{euclid\_sentence} rather than \texttt{have} to show the mapping from the \NL sentence $s_1=\text{"For if $AB$... greater."}$ to its formal counterpart $\formal{\assert{s_1}}=|(a\--b)| > |(a\--c)| \lor |(a\--c)| > |(a\--b)|$ and $\formal{\assumptions{s_1}}=\{|(a\--b)| \neq |(a\--c)|\}$.
  \texttt{euclid\_sentence} behaves in the same way as \texttt{have} except it embeds one extra string input to define the structural mapping from the \NL sentence to its formal code.
}
\label{fig:segment}
\end{figure*}


==> figures/fig-segment.tex <==
% =====================================================================
% Small example: a single faithful segment (Book I, Prop 6, step 1).
% A full-column-width framed lstlisting inside a figure float, so the
% code fills the column instead of leaving a blank right strip.
% Font is shrunk with tight line spacing so each statement sits on its
% own line without wrapping.  Source: My_Prop06/Main.lean, step 1.
% =====================================================================
\begin{figure*}[t]
\centering
\input{figures/fig-segment-body.tex}
\caption{
  A single \emph{faithful segment}: Euclid's sentence \smark{1} of Prop.~6, expanding from the same Prop~6 example from \cref{fig:motivation} which was a \emph{simplification}.
  This example uses \texttt{euclid\_segment} rather than \texttt{have} to show the mapping from the \NL sentence $s_1=\text{"For if $AB$... greater."}$ to its formal counterpart $\formal{\assert{s_1}}=|(a\--b)| > |(a\--c)| \lor |(a\--c)| > |(a\--b)|$ and $\formal{\assumptions{s_1}}=\{|(a\--b)| \neq |(a\--c)|\}$.
  \texttt{euclid\_segment} behaves in the same way as \texttt{have} except it embeds one extra string input to define the structural mapping from the \NL sentence to its formal code.
}
\label{fig:segment}
\end{figure*}


==> sections/1-abs-submit.tex <==
In formal verification, both the autoformalization of statements and automated proof search have been studied extensively. While automated proof search can produce a formal proof that compiles, the generated proof does not necessarily reflect how the natural-language argument arrives at its conclusion—a property we refer to as faithfulness. With faithfully formalized proofs, one can check the reasoning behind a human- or AI-written argument, and assist mathematicians in formalizing their proof sketches. However, it is particularly challenging due to misalignment of formal proof tactics and natural language reasoning. In this work, we rigorously describe a set of five necessary conditions a faithful formal proof must satisfy, and introduce Pistis, an agentic, oracle-guided proof search that produces formal Lean proofs that provably satisfy them. At its core is a novel faithfulness-preserving divide-and-conquer search, which we name OrderDecompose, that tracks citation dependencies and blocks unfaithful shortcuts, paired with a refutation search, that surfaces gaps and errors in the natural language proof source. OrderDecompose completes proofs that baselines cannot close even within a 12-hour budget, and its artifacts compile over 33× as fast as prior work's. We apply Pistis on the first three books of Euclid's Elements, producing high-quality artifacts containing faithful formal proofs. Under a blinded human study and an LLM-as-a-judge protocol on rigorous rubrics, Pistis-generated proofs are favored over prior works—2.89× and 5.2× as often by human reviewers and the LLM judge, respectively. It further uncovers gaps in Euclid's proofs and their translation, and can accept or refute natural language proofs written by humans or AI, demonstrating that faithful formalization is useful as a proof-checking tool.

